Cdh descent in equivariant homotopy K-theory

We construct geometric models for classifying spaces of linear algebraic groups in G-equivariant motivic homotopy theory, where G is a tame group scheme. As a consequence, we show that the equivariant motivic spectrum representing the homotopy K-theory of G-schemes (which we construct as an E-infinity-ring) is stable under arbitrary base change, and we deduce that homotopy K-theory of G-schemes satisfies cdh descent.

==> tikzlibrarydiagrams.code.tex <==
\usetikzlibrary{matrix,arrows,decorations}

\makeatletter
\def\@tipextend{
	\arrowsize=.3pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-3\arrowsize-.5\pgflinewidth}
	\pgfarrowsrightextend{.5\pgflinewidth}
}
\def\@tipoptions{
	\pgfsetdash{}{0pt}
	\pgfsetroundcap
	\pgfsetroundjoin
}

\pgfarrowsdeclare{tip}{tip}{\@tipextend}{
	\@tipoptions
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-3.5\pgfutil@tempdima}{6.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-2.8\pgfutil@tempdima}{2\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-2.8\pgfutil@tempdima}{-2\pgfutil@tempdima}}
	               {\pgfpoint{-3.5\pgfutil@tempdima}{-6.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\pgfarrowsdeclare{top}{top}{\@tipextend}{
	\@tipoptions
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-3.5\pgfutil@tempdima}{6.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-2.8\pgfutil@tempdima}{2\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-1.95\pgfutil@tempdima}{-1.8\pgfutil@tempdima}}
	               {\pgfpoint{-2.85\pgfutil@tempdima}{-4.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\pgfarrowsdeclare{bot}{bot}{\@tipextend}{
	\@tipoptions 
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-2.85\pgfutil@tempdima}{4.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-1.95\pgfutil@tempdima}{1.8\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-2.8\pgfutil@tempdima}{-2\pgfutil@tempdima}}
	               {\pgfpoint{-3.5\pgfutil@tempdima}{-6.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\pgfarrowsdeclare{mid}{mid}{\@tipextend}{
	\@tipoptions 
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-2.85\pgfutil@tempdima}{4.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-1.95\pgfutil@tempdima}{1.8\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-1.95\pgfutil@tempdima}{-1.8\pgfutil@tempdima}}
	               {\pgfpoint{-2.85\pgfutil@tempdima}{-4.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}

\expandafter\let\csname pgf@ar@means@|\endcsname=\relax
\expandafter\let\csname pgf@arrow@code@|\endcsname=\relax
\pgfarrowsdeclare{|}{|}{
	\pgfarrowsleftextend{-0.25\pgflinewidth}
	\pgfarrowsrightextend{.75\pgflinewidth}
}{
	\@tipoptions 
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{0pt}{6\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{0pt}{-6\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\makeatother

\pgfdeclaredecoration{normal}{initial}{
	\state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfpathmoveto{\pgfpointorigin}} 
	\state{final}{\pgfpathlineto{\pgfpointorigin}} 
}

\pgfarrowsdeclarealias{c}{c}{left hook}{right hook}

% Variables settable at the beginning of tikzpicture environment
\def\rowsep{2.5em}
\def\colsep{2.5em}

% Distance between double arrows is 2\dbl
\def\dbl{1.7}

\def\diagram{\matrix[diagram]}
\def\arrows{\path[->,font=\scriptsize]}

\newenvironment{tikzcentered}{\center\tikzpicture}{\endtikzpicture\endcenter}
\newenvironment{tikzmath}{\displaymath\tikzpicture}{\endtikzpicture\enddisplaymath}
\newenvironment{tikzequation}{\equation\tikzpicture}{\endtikzpicture\endequation}

\tikzset{
	every picture/.style={
		baseline=(current bounding box.center),% equation numbers are centered.
		>=tip,% set default arrow tip
		line cap=round % set round caps
	},
	diagram/.style={
		inner sep=0,% we don't want any additional margin for diagrams (displaymath/center takes care of that)
		execute at begin cell=\node\bgroup\math\displaystyle,% displaystyle math nodes
		execute at end cell={
			\endmath\egroup;% close node
			\coordinate (-\the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn) at ([yshift=2.6] \the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn.base west);% set uniform left horizontal anchor
			\coordinate (\the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn -) at ([yshift=2.6] \the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn.base east);% set uniform right horizontal anchor
		},
		cells={anchor=base},% aligns text across cells
		nodes={
			name=\the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn,% name (ij)
			inner sep=.3333em % default padding (override the matrix's 'inner sep=0')
		},
		row sep=\rowsep,
		column sep=\colsep
	},
	vshift/.style={
		decoration={normal,raise=#1},
		decorate 
	}
}
